Translation of Multifaceted Data without Re-Training of Machine Translation Systems

Translating major language resources to build minor language resources becomes a widely-used approach. Particularly in translating complex data points composed of multiple components, it is common to translate each component separately. However, we argue that this practice often overlooks the interrelation between components within the same data point. To address this limitation, we propose a novel MT pipeline that considers the intra-data relation in implementing MT for training data. In our MT pipeline, all the components in a data point are concatenated to form a single translation sequence and subsequently reconstructed to the data components after translation. We introduce a Catalyst Statement (CS) to enhance the intra-data relation, and Indicator Token (IT) to assist the decomposition of a translated sequence into its respective data components. Through our approach, we have achieved a considerable improvement in translation quality itself, along with its effectiveness as training data. Compared with the conventional approach that translates each data component separately, our method yields better training data that enhances the performance of the trained model by 2.690 points for the web page ranking (WPR) task, and 0.845 for the question generation (QG) task in the XGLUE benchmark.

==> sections/A.Downstream_Task_Performance.tex <==
\input{Tables/Table_performance_full}
In Table~\ref{tb:performance_all}, the performance of the downstream task according to each translation model is presented. Interestingly, despite always training with fewer data, our approach consistently demonstrates superior performance to that of the conventional Separate translation method in all cases. Furthermore, in WPR, which encompasses more data components than QG, we achieve an average gain of more than 2 points. Since having a multitude of components implies a stronger intra-relation within the data, the consideration of relation in dataset with more components induces a significant difference in performance.

Moreover, even if RP is not employed, our performance consistently exceeds that of Separate. The introduction of IT induces the consideration of inter-component relations that are unidentifiable when the data components are translated individually. However, most cases exhibit the highest performance when a relation considered RP is employed. This suggests that our method is straightforward yet effective in producing high-quality training data, considering the aim to enhance the model's other linguistic capabilities.


% In Table~\ref{tb:performance_all}, the performance of the downstream task is presented according to each translation model. Surprisingly, Separate 보다 항상 적은 수의 데이터가 학습됨에도 불구하고, our method demonstrates superior performance in all possible cases when compared to the ordinary translation method (Separate). 또한, QG보다 더 많은 data component를 갖는 WPR에서는 평균적으로 약 2점 이상의 gain을 얻는다. 다수의 components는 data 내의 intra-relation이 더 강하다는 것을 의미하기 때문에 관계성의 고려는 성능에서 더 큰 차이를 야기한다.

% 또한 CP를 사용하지 않았을때 조차 Separate보다 성능이 항상 높은데, 이는 Indicator token의 도입이 data components가 각각 번역되었을때는 파악할 수 없는 component간의 관계를 고려하게 끔 유도하고 있음을 의미한다. 또한 Relation이 고려된 CP를 사용하는 경우 대부분의 경우에서 성능이 가장 높다. 이는 우리의 방법이 모델의 다른 언어능력을 증대시키고자하는 목적을 고려할때 우수한 학습데이터를 생산하는데 단순하면서도 효과적이라는 것을 시사한다.
